Is Attention Interpretation? A Quantitative Assessment On Sets

The debate around the interpretability of attention mechanisms is centered on whether attention scores can be used as a proxy for the relative amounts of signal carried by sub-components of data. We propose to study the interpretability of attention in the context of set machine learning, where each data point is composed of an unordered collection of instances with a global label. For classical multiple-instance-learning problems and simple extensions, there is a well-defined "importance" ground truth that can be leveraged to cast interpretation as a binary classification problem, which we can quantitatively evaluate. By building synthetic datasets over several data modalities, we perform a systematic assessment of attention-based interpretations. We find that attention distributions are indeed often reflective of the relative importance of individual instances, but that silent failures happen where a model will have high classification performance but attention patterns that do not align with expectations. Based on these observations, we propose to use ensembling to minimize the risk of misleading attention-based explanations.

==> accuracy_vs_auroc_whole_hps.tex <==
\begin{figure}[h]
\begin{multicols}{2}
  \centering
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\textwidth]{figures/gaussian_mil/whole_hps/accuracy_vs_auroc_customheat.pdf}
\caption{Gaussian MIL\label{fig:acc_vs_auroc_mil}}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\textwidth]{figures/gaussian_and/whole_hps/accuracy_vs_auroc_customheat.pdf}
\caption{Gaussian AND\label{fig:acc_vs_auroc_and}}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\textwidth]{figures/gaussian_xor/whole_hps/accuracy_vs_auroc_customheat.pdf}
\caption{Gaussian XOR\label{fig:acc_vs_auroc_xor}}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\textwidth]{figures/mnist_mil/whole_hps/accuracy_vs_auroc_customheat.pdf}
\caption{MNIST MIL\label{fig:acc_vs_auroc_mnist_mil}}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\textwidth]{figures/mnist_and/whole_hps/accuracy_vs_auroc_customheat.pdf}
\caption{MNIST AND\label{fig:acc_vs_auroc_mnist_and}}
\end{subfigure}
\begin{subfigure}{0.23\textwidth}
\includegraphics[width=\textwidth]{figures/mnist_xor/whole_hps/accuracy_vs_auroc_customheat.pdf}
\caption{MNIST XOR\label{fig:acc_vs_auroc_mnist_xor}}
\end{subfigure}
\end{multicols}

\caption{Relationship between validation accuracy and test importance attribution AUROC for whole hyperparameter search \label{fig:acc_vs_auroc_whole_hps}}
\end{figure}

==> dump.tex <==
% stuff to delete eventually

In order to confront the model's attention pattern to strict ground truth, we defined different rules dictating the bag label based on the instances the bag contains and generated datasets following those rules.
In the classical MIL setup for instance, the bags can be either negative and positive. Negative bags only contain negative instances whereas positive bags contain at least one positive instance.
In addition to this typical case, we explored datasets governed by the AND and XOR logical rules. 
In those more complicated cases, the bags contained up to three populations, one of which served as background whereas the (simultaneous) presence of the two other populations induces the bag label.
In other words, given a bag of instances $X = \{x_1, x_2, ..., x_M\}$ where each instance is assumed to be associated with a label $y_m$ where $1 < m < M$, the bag label $Y$ is:

\noindent
\textbf{MIL}
\begin{itemize}
    \item[] $y_m \in \{0, 1\}$ 
    \item[] $m \in [1, M]$
    \item[] $Y = \begin{cases}
1 \quad \text{if} \quad \exists \quad m \quad | \quad y_m = 1 \\
0 \quad \text{otherwise}
\end{cases}
$
\end{itemize}

\vspace{.3cm}
\noindent
\textbf{AND}
\begin{itemize}
    \item[] $y_m \in \{0, 1, 2\}$ 
    \item[] $m, n \in [1, M]$
    \item[] $Y = \begin{cases}
1 \quad \text{if} \quad \exists \quad m, n \quad | \quad y_m = 1, \quad y_n = 2 \\
0 \quad \text{otherwise}
\end{cases}
$
\end{itemize}

\vspace{.3cm}
\noindent
\textbf{XOR}
\begin{itemize}
    \item[] $y_m \in \{0, 1, 2\}$ 
    \item[] $m, n \in [1, M]$
    \item[] $Y = \begin{cases}
1 \quad \text{if} \quad \exists \quad m, \quad \nexists \quad n \quad | \quad y_m = 1, \quad y_n = 2  \\
1 \quad \text{if} \quad \nexists \quad m, \quad \exists \quad n \quad | \quad y_m = 1, \quad y_n = 2  \\
%1 \quad \text{if} \quad \exists \quad m, n \in [1, M] \quad | \quad y_m = 1 \veebar y_n = 2 \\
0 \quad \text{otherwise}
\end{cases}
$
\end{itemize}
